Sim-to-Real Model-Based and Model-Free Deep Reinforcement Learning for Tactile Pushing

Object pushing presents a key non-prehensile manipulation problem that is illustrative of more complex robotic manipulation tasks. While deep reinforcement learning (RL) methods have demonstrated impressive learning capabilities using visual input, a lack of tactile sensing limits their capability for fine and reliable control during manipulation. Here we propose a deep RL approach to object pushing using tactile sensing without visual input, namely tactile pushing. We present a goal-conditioned formulation that allows both model-free and model-based RL to obtain accurate policies for pushing an object to a goal. To achieve real-world performance, we adopt a sim-to-real approach. Our results demonstrate that it is possible to train on a single object and a limited sample of goals to produce precise and reliable policies that can generalize to a variety of unseen objects and pushing scenarios without domain randomization. We experiment with the trained agents in harsh pushing conditions, and show that with significantly more training samples, a model-free policy can outperform a model-based planner, generating shorter and more reliable pushing trajectories despite large disturbances. The simplicity of our training environment and effective real-world performance highlights the value of rich tactile information for fine manipulation. Code and videos are available at https://sites.google.com/view/tactile-rl-pushing/.

==> math/rap2texdefs.tex <==
%% rap2texdefs.tex
%
% A file containing LaTeX command definitions
% used in mathematical documents.

\usepackage{amsmath,amsfonts,amssymb}

%\newtheorem{theorem}{Theorem}
%\newtheorem{axiom}[theorem]{Axiom}
%\newtheorem{corollary}[theorem]{Corollary}
%\newtheorem{definition}[theorem]{Definition}
%\newtheorem{fact}[theorem]{Fact}
%\newtheorem{facts}{Facts}
%\newtheorem{lemma}[theorem]{Lemma}
%\newtheorem{note}{Note}
%\newtheorem{notes}{Notes}
%\newtheorem{proposition}[theorem]{Proposition}

% \DeclareMathOperator requires \usepackage{amsmath}
\DeclareMathOperator{\Adj}{adj}
\DeclareMathOperator{\mAnd}{and}
\DeclareMathOperator{\AND}{AND}
\DeclareMathOperator*{\Argmin}{argmin}
\DeclareMathOperator*{\Argmax}{argmax}
\DeclareMathOperator{\Char}{char}
\DeclareMathOperator{\Cod}{cod}
\DeclareMathOperator{\Deg}{deg}
\DeclareMathOperator{\Dom}{dom}
\DeclareMathOperator{\Diag}{diag}
%\DeclareMathOperator{\If}{if}
\DeclareMathOperator{\Imag}{Im}
\DeclareMathOperator{\Or}{or}
\DeclareMathOperator{\OR}{OR}
\DeclareMathOperator*{\Med}{med}
\DeclareMathOperator{\Null}{null}
\DeclareMathOperator{\Nullity}{nullity}
\DeclareMathOperator{\Range}{range}
\DeclareMathOperator{\Rank}{rank}
\DeclareMathOperator{\Real}{Re}
\DeclareMathOperator{\Sgn}{sgn}
\DeclareMathOperator{\Sinc}{sinc}
\DeclareMathOperator{\Span}{span}
\DeclareMathOperator{\Tr}{Tr}
\DeclareMathOperator{\Where}{where}



\newcommand{\ti}[1]{\mbox{\tiny $#1$}}
\newcommand{\st}[1]{\mbox{\scriptsize $#1$}}
\newcommand{\fn}[1]{\mbox{\footnotesize $#1$}}
\newcommand{\sm}[1]{\mbox{\small $#1$}}
\newcommand{\ns}[1]{\mbox{\normalsize $#1$}}
\newcommand{\la}[1]{\mbox{\large $#1$}}
\newcommand{\La}[1]{\mbox{\Large $#1$}}
\newcommand{\LA}[1]{\mbox{\LARGE $#1$}}
\newcommand{\hu}[1]{\mbox{\huge $#1$}}
\newcommand{\Hu}[1]{\mbox{\Huge $#1$}}
\newcommand{\blds}[1]{\mbox{\scriptsize \boldmath $#1$}}

\newcommand{\BI}[1]{\textbf{\emph {#1}}}
\newcommand{\I}[1]{\emph {#1}}

\newcommand{\ie}{{\em i.e.}}
\newcommand{\Ie}{{\em I.e.}}
\newcommand{\eg}{{\em e.g.}}
\newcommand{\Eg}{{\em E.g.}}
\newcommand{\et}{{\em et al.}}
\newcommand{\vs}{{\em vs.\ }}

\newcommand{\lip}{\mbox{$\langle$}}
\newcommand{\rip}{\mbox{$\rangle$}}
\newcommand{\Lip}{\left\langle}
\newcommand{\Rip}{\right\rangle}

\newcommand{\lar}{\mbox{$\;\,\leftarrow\;\,$}}
\newcommand{\rar}{\mbox{$\;\,\rightarrow\;\,$}}
\newcommand{\Lar}{\mbox{$\;\,\Leftarrow\;\,$}}
\newcommand{\Rar}{\mbox{$\;\,\Rightarrow\;\,$}}
\newcommand{\lrar}{\mbox{$\;\,\leftrightarrow\;\,$}}
\newcommand{\LRar}{\mbox{$\;\,\Leftrightarrow\;\,$}}

\newcommand{\vareps}{\mbox{$\varepsilon$}}

\newcommand{\Ob}{\mbox{$\bf 0$}}
\newcommand{\ab}{\mbox{$\bf a$}}
\newcommand{\bb}{\mbox{$\bf b$}}
\newcommand{\cb}{\mbox{$\bf c$}}
\newcommand{\db}{\mbox{$\bf d$}}
\newcommand{\eb}{\mbox{$\bf e$}}
\newcommand{\fb}{\mbox{$\bf f$}}
\newcommand{\gb}{\mbox{$\bf g$}}
\newcommand{\hb}{\mbox{$\bf h$}}
\newcommand{\ib}{\mbox{$\bf i$}}
\newcommand{\jb}{\mbox{$\bf j$}}
\newcommand{\kb}{\mbox{$\bf k$}}
\newcommand{\lb}{\mbox{$\bf l$}}
\newcommand{\mb}{\mbox{$\bf m$}}
\newcommand{\nb}{\mbox{$\bf n$}}
\newcommand{\ob}{\mbox{$\bf o$}}
\newcommand{\pb}{\mbox{$\bf p$}}
\newcommand{\qb}{\mbox{$\bf q$}}
\newcommand{\rb}{\mbox{$\bf r$}}
\newcommand{\sbf}{\mbox{$\bf s$}}
\newcommand{\tb}{\mbox{$\bf t$}}
\newcommand{\ub}{\mbox{$\bf u$}}
\newcommand{\vb}{\mbox{$\bf v$}}
\newcommand{\wb}{\mbox{$\bf w$}}
\newcommand{\xb}{\mbox{$\bf x$}}
\newcommand{\yb}{\mbox{$\bf y$}}
\newcommand{\zb}{\mbox{$\bf z$}}

\newcommand{\alpb}{\mbox{$\vec{\alpha}$}}
\newcommand{\betb}{\mbox{$\vec{\beta}$}}
\newcommand{\gamb}{\mbox{$\vec{\gamma}$}}
\newcommand{\delb}{\mbox{$\vec{\delta}$}}
\newcommand{\epsb}{\mbox{$\vec{\epsilon}$}}
\newcommand{\rhob}{\mbox{$\vec{\rho}$}}
\newcommand{\theb}{\mbox{$\vec{\theta}$}}

\newcommand{\AB}{\mbox{$\bf A$}}
\newcommand{\BB}{\mbox{$\bf B$}}
\newcommand{\CB}{\mbox{$\bf C$}}
\newcommand{\DB}{\mbox{$\bf D$}}
\newcommand{\EB}{\mbox{$\bf E$}}
\newcommand{\FB}{\mbox{$\bf F$}}
\newcommand{\GB}{\mbox{$\bf G$}}
\newcommand{\HB}{\mbox{$\bf H$}}
\newcommand{\IB}{\mbox{$\bf I$}}
\newcommand{\JB}{\mbox{$\bf J$}}
\newcommand{\KB}{\mbox{$\bf K$}}
\newcommand{\LB}{\mbox{$\bf L$}}
\newcommand{\MB}{\mbox{$\bf M$}}
\newcommand{\NB}{\mbox{$\bf N$}}
\newcommand{\OB}{\mbox{$\bf O$}}
\newcommand{\PB}{\mbox{$\bf P$}}
\newcommand{\QB}{\mbox{$\bf Q$}}
\newcommand{\RB}{\mbox{$\bf R$}}
\newcommand{\SB}{\mbox{$\bf S$}}
\newcommand{\TB}{\mbox{$\bf T$}}
\newcommand{\UB}{\mbox{$\bf U$}}
\newcommand{\VB}{\mbox{$\bf V$}}
\newcommand{\WB}{\mbox{$\bf W$}}
\newcommand{\XB}{\mbox{$\bf X$}}
\newcommand{\YB}{\mbox{$\bf Y$}}
\newcommand{\ZB}{\mbox{$\bf Z$}}

\newcommand{\AC}{\mbox{$\mathcal A$}}
\newcommand{\BC}{\mbox{$\mathcal B$}}
\newcommand{\CC}{\mbox{$\mathcal C$}}
\newcommand{\DC}{\mbox{$\mathcal D$}}
\newcommand{\EC}{\mbox{$\mathcal E$}}
\newcommand{\FC}{\mbox{$\mathcal F$}}
\newcommand{\GC}{\mbox{$\mathcal G$}}
\newcommand{\HC}{\mbox{$\mathcal H$}}
\newcommand{\IC}{\mbox{$\mathcal I$}}
\newcommand{\JC}{\mbox{$\mathcal J$}}
\newcommand{\KC}{\mbox{$\mathcal K$}}
\newcommand{\LC}{\mbox{$\mathcal L$}}
\newcommand{\MC}{\mbox{$\mathcal M$}}
\newcommand{\NC}{\mbox{$\mathcal N$}}
\newcommand{\OC}{\mbox{$\mathcal O$}}
\newcommand{\PC}{\mbox{$\mathcal P$}}
\newcommand{\QC}{\mbox{$\mathcal Q$}}
\newcommand{\RC}{\mbox{$\mathcal R$}}
\newcommand{\SC}{\mbox{$\mathcal S$}}
\newcommand{\TC}{\mbox{$\mathcal T$}}
\newcommand{\UC}{\mbox{$\mathcal U$}}
\newcommand{\VC}{\mbox{$\mathcal V$}}
\newcommand{\WC}{\mbox{$\mathcal W$}}
\newcommand{\XC}{\mbox{$\mathcal X$}}
\newcommand{\YC}{\mbox{$\mathcal Y$}}
\newcommand{\ZC}{\mbox{$\mathcal Z$}}

\newcommand{\CF}{\mbox{$\mathbb{C}$}}
\newcommand{\FF}{\mbox{$\mathbb{F}$}}
\newcommand{\MF}{\mbox{$\mathbb{M}$}}
\newcommand{\NF}{\mbox{$\mathbb{N}$}}
\newcommand{\QF}{\mbox{$\mathbb{Q}$}}
\newcommand{\RF}{\mbox{$\mathbb{R}$}}
\newcommand{\WF}{\mbox{$\mathbb{W}$}}
\newcommand{\ZF}{\mbox{$\mathbb{Z}$}}

\newcommand{\ac}{\mbox{$\check{\bf a}$}}
\newcommand{\ah}{\mbox{$\hat{\bf a}$}}
\newcommand{\app}{\mbox{${\bf a}^{\perp}$}}
\newcommand{\apr}{\mbox{${\bf a}^{\prime}$}}

\newcommand{\bc}{\mbox{$\check{\bf b}$}}
\newcommand{\bh}{\mbox{$\hat{\bf b}$}}
\newcommand{\bpp}{\mbox{${\bf b}^{\perp}$}}
\newcommand{\bpr}{\mbox{${\bf b}^{\prime}$}}

\newcommand{\cc}{\mbox{$\check{\bf c}$}}
\newcommand{\ch}{\mbox{$\hat{\bf wc}$}}
\newcommand{\cpp}{\mbox{${\bf c}^{\perp}$}}
\newcommand{\cpr}{\mbox{${\bf c}^{\prime}$}}

\newcommand{\ic}{\mbox{$\check{\bf i}$}}
\newcommand{\ih}{\mbox{$\hat{\bf i}$}}
\newcommand{\ipp}{\mbox{${\bf i}^{\perp}$}}
\newcommand{\idpr}{\mbox{${\bf i}^{\prime}$}}

\newcommand{\jc}{\mbox{$\check{\bf j}$}}
\newcommand{\jh}{\mbox{$\hat{\bf j}$}}
\newcommand{\jpp}{\mbox{${\bf j}^{\perp}$}}
\newcommand{\jpr}{\mbox{${\bf j}^{\prime}$}}

\newcommand{\kc}{\mbox{$\check{\bf k}$}}
\newcommand{\kh}{\mbox{$\hat{\bf k}$}}
\newcommand{\kpp}{\mbox{${\bf k}^{\perp}$}}
\newcommand{\kpr}{\mbox{${\bf k}^{\prime}$}}

\newcommand{\uc}{\mbox{$\check{\bf u}$}}
\newcommand{\uh}{\mbox{$\hat{\bf u}$}}
\newcommand{\upp}{\mbox{${\bf u}^{\perp}$}}
\newcommand{\upr}{\mbox{${\bf u}^{\prime}$}}

\newcommand{\vc}{\mbox{$\check{\bf v}$}}
\newcommand{\vh}{\mbox{$\hat{\bf v}$}}
\newcommand{\vpp}{\mbox{${\bf v}^{\perp}$}}
\newcommand{\vpr}{\mbox{${\bf v}^{\prime}$}}

\newcommand{\wc}{\mbox{$\check{\bf w}$}}
\newcommand{\wh}{\mbox{$\hat{\bf w}$}}
\newcommand{\wpp}{\mbox{${\bf w}^{\perp}$}}
\newcommand{\wpr}{\mbox{${\bf w}^{\prime}$}}

\newcommand{\xc}{\mbox{$\check{\bf x}$}}
\newcommand{\xh}{\mbox{$\hat{\bf x}$}}
\newcommand{\xpp}{\mbox{${\bf x}^{\perp}$}}
\newcommand{\xpr}{\mbox{${\bf x}^{\prime}$}}

\newcommand{\yc}{\mbox{$\check{\bf y}$}}
\newcommand{\yh}{\mbox{$\hat{\bf y}$}}
\newcommand{\ypp}{\mbox{${\bf y}^{\perp}$}}
\newcommand{\ypr}{\mbox{${\bf y}^{\prime}$}}

\newcommand{\zc}{\mbox{$\check{\bf z}$}}
\newcommand{\zh}{\mbox{$\hat{\bf z}$}}
\newcommand{\zpp}{\mbox{${\bf z}^{\perp}$}}
\newcommand{\zpr}{\mbox{${\bf z}^{\prime}$}}

\newcommand{\ol}[1]{\overline{#1}}
\newcommand{\bs}{\mbox{$\backslash$}}
\newcommand{\nin}{\noindent}
\newcommand{\vsni}{\vspace{1em} \noindent}
\newcommand{\nn}{\nonumber}

\newcommand{\beq}{\begin{equation}}
\newcommand{\eeq}{\end{equation}}
\newcommand{\bear}{\begin{eqnarray}}
\newcommand{\bears}{\begin{eqnarray*}}
\newcommand{\eear}{\end{eqnarray}}
\newcommand{\eears}{\end{eqnarray*}}
\newcommand{\bdm}{\begin{displaymath}}
\newcommand{\edm}{\end{displaymath}}
\newcommand{\lba}{\left[\begin{array}}
\newcommand{\ear}{\end{array}\right]}

\newcommand{\eqdef}{\stackrel{\rm def}{=}}
\newcommand{\tdot}[1]{\stackrel{\ldots}{#1}}

\newcommand{\priori}{\emph{a priori}}
\newcommand{\degree}{^\circ} 
